Penalized Semidefinite Programming for Quadratically-Constrained Quadratic Optimization

In this paper, we give a new penalized semidefinite programming approach for non-convex quadratically-constrained quadratic programs (QCQPs). We incorporate penalty terms into the objective of convex relaxations in order to retrieve feasible and near-optimal solutions for non-convex QCQPs. We introduce a generalized linear independence constraint qualification (GLICQ) criterion and prove that any GLICQ regular point that is sufficiently close to the feasible set can be used to construct an appropriate penalty term and recover a feasible solution. Inspired by these results, we develop a heuristic sequential procedure that preserves feasibility and aims to improve the objective value at each iteration. Numerical experiments on large-scale system identification problems as well as benchmark instances from the library of quadratic programming (QPLIB) demonstrate the ability of the proposed penalized semidefinite programs in finding near-optimal solutions for non-convex QCQP.

==> plot_01.tex <==
%%%%%%%%% ABSTRACT
\tikzset{
	master/.style={
		execute at end picture={
			\coordinate (lower right) at (current bounding box.south east);
			\coordinate (upper left) at (current bounding box.north west);
		}
	},
	slave/.style={
		execute at end picture={
			\pgfresetboundingbox
			\path (upper left) rectangle (lower right);
		}
	}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\captionsetup[subfigure]{position=t}
\centering
\begin{tikzpicture}[master,scale=1]
\centering
%\tikzstyle{every node}=[font=\large]
\begin{axis}[
		width = 0.48\textwidth,
		height = 0.28\textwidth,
 		xmode=normal,
		ymode=log,	
%     	xlabel={\large$\mu$},
    	ylabel={$\mathrm{tr}\{\mathbf{X}-\mathbf{x}\mathbf{x}^{\!_\top}\!\}$},
    	ylabel shift =0cm,
  		xmin=0,
 	 	xmax=50,
%       xtickmax = 7500,
%		ymin=1e-5, 
% 	 	ymax= 50,
%   	xtick={0,100,200,300,400},
%   	ytick={1e-6, 1e-5, 1e-4, 1e-3, 1e-2, 1e-1},
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\eta \times 10^{-\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
% 		scaled x ticks = base 10:-3,
    	legend pos=north east,
    	ymajorgrids=true,
		xmajorgrids=true,
    	grid style=dashed,
		legend cell align={left},
        legend image post style={scale=0.5},
        legend style={font=\scriptsize, inner xsep=0.2pt, inner ysep=0.1pt,at={(axis cs:49.5,0.30)}},
]
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:7.70282,4)--(axis cs:49.9,4) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:18.534,0.8)--(axis cs:49.9,0.8) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:1.96499,2.5)--(axis cs:49.9,2.5) node [black, pos=0.5, below] {\footnotesize \raisebox{-0.5ex}[1.4pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
%==================
\addplot[color=blue,line width=0.5mm] table[x=mu,y=infsSDPlbub,col sep=comma] {data.csv};
\addplot[dashed,color=red,line width=0.5mm] table[x=mu,y=infsSOCPlbub,col sep=comma] {data.csv};
\addplot[dash dot,color=black,line width=0.5mm] table[x=mu,y=infsSDPRLTlbub,col sep=comma] {data.csv};
%===================
\legend{$\mathrm{SDP}$,$\mathrm{SOCP}$,$\mathrm{SDP\!+\!RLT}$}
% \addplot[dashed, color=red,line width=0.5mm] table[x=X,y=Y2,col sep=comma] {Results/testdataErr.csv};
% \legend{$\mu=0.1$, $\mu=1$, $\mu=10$}
\end{axis}
\end{tikzpicture}
\vspace{0.2cm}
\begin{tikzpicture}[slave,scale=1]
\centering
\begin{axis}[
		width = 0.48\textwidth,
		height = 0.28\textwidth,
 		xmode=normal,
%       xmode=log,
		ymode=normal,	
        xlabel={\large$\eta$},
        ylabel={$q_0(\boldsymbol{x})$},
		ylabel shift = 0cm,
  		xmin=0,
   		xmax=50,
%     	ymin = 10.0,
%      	ymax = 11.5,
%       ytickmax = 11.4,,
%       xtickmax = 7500,
%    xtick={0,2000,4000,6000,,8000},
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\eta \times 10^{-\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
% 		scaled x ticks = base 10:-3,
% 		ytick={10.00, 10.25, 10.50, 10.75, 11.00, 11.25, 11.50},
%     	yticklabels={~, 10.25, 10.50, 10.75, 11.00, 11.25, 11.50},
    	legend pos= south east,
    	ymajorgrids=true,
		xmajorgrids=true,
    	grid style=dashed,
		legend cell align={left},
        legend image post style={scale=0.5},
        legend style={font=\scriptsize, inner xsep=0.2pt, inner ysep=0.1pt,at={(axis cs:49.5,-52)}},
]
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:7.70282,-26.158)--(axis cs:49.9,-26.158) node [black, pos=0.5, above] {\small \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:18.53,-14.13455)--(axis cs:49.9,-14.13455) node [black, pos=0.6, above] {\small \raisebox{-0.5ex}[2pt][-1ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:1.976,-58.761)--(axis cs:49.9,-58.761) node [black, pos=0.5, above] {\small \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
%=========================
\addplot[color=blue,line width=0.5mm] table[x=mu,y=objSDPlbub,col sep=comma] {data.csv};
\addplot[dashed,color=red,line width=0.5mm] table[x=mu,y=objSOCPlbub,col sep=comma] {data.csv};
\addplot[dash dot,color=black,line width=0.5mm] table[x=mu,y=objSDPRLTlbub,col sep=comma] {data.csv};
\legend{$\mathrm{SDP}$,$\mathrm{SOCP}$,$\mathrm{SDP\!+\!RLT}$}
%========================
\end{axis}
\end{tikzpicture}
\vspace{-2mm}
\caption{Sensitivity of the penalized SDP, SOCP, and SDP+RLT relaxations to the choice of penalty parameter $\eta$ for the QCQP benchmark case 1143 and $\hat{\boldsymbol{x}}=\boldsymbol{x}^{\mathrm{flat}}$.}
\label{plt:lbub}
\end{figure}


==> plot_02.tex <==
%%%%%%%%% ABSTRACT
\tikzset{
	master/.style={
		execute at end picture={
			\coordinate (lower right) at (current bounding box.south east);
			\coordinate (upper left) at (current bounding box.north west);
		}
	},
	slave/.style={
		execute at end picture={
			\pgfresetboundingbox
			\path (upper left) rectangle (lower right);
		}
	}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\captionsetup[subfigure]{position=b}
\centering
\begin{tikzpicture}[master,scale=1]
\centering
%\tikzstyle{every node}=[font=\large]
\begin{axis}[
		width = 0.48\textwidth,
		height = 0.28\textwidth,
 		xmode=normal,
		ymode=log,	
%     	xlabel={\large$\mu$},
    	ylabel={$\mathrm{tr}\{\mathbf{X}-\mathbf{x}\mathbf{x}^{\!_\top}\!\}$},
    	ylabel shift =0cm,
  		xmin=0,
 	 	xmax=50,
%       xtickmax = 7500,
%		ymin=1e-5, 
% 	 	ymax= 50,
%   	xtick={0,100,200,300,400},
%   	ytick={1e-6, 1e-5, 1e-4, 1e-3, 1e-2, 1e-1},
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\eta \times 10^{-\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
% 		scaled x ticks = base 10:-3,
    	legend pos=north east,
    	ymajorgrids=true,
		xmajorgrids=true,
    	grid style=dashed,
		legend cell align={left},
        legend image post style={scale=0.5},
        legend style={font=\scriptsize, inner xsep=0.2pt, inner ysep=0.1pt,at={(axis cs:49.5,0.3)}},
]
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:7.5,4.0)--(axis cs:49.9,4.0) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:21.434,0.65)--(axis cs:49.9,0.65) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:0.958425,1.2)--(axis cs:49.9,1.2) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
%==================
\addplot[color=blue,line width=0.5mm] table[x=mu,y=infsSDPsdprlt,col sep=comma] {data.csv};
\addplot[dashed,color=red,line width=0.5mm] table[x=mu,y=infsSOCPsdprlt,col sep=comma] {data.csv};
\addplot[dash dot,color=black,line width=0.5mm] table[x=mu,y=infsSDPRLTsdprlt,col sep=comma] {data.csv};
%===================
\legend{$\mathrm{SDP}$,$\mathrm{SOCP}$,$\mathrm{SDP\!+\!RLT}$}
% \addplot[dashed, color=red,line width=0.5mm] table[x=X,y=Y2,col sep=comma] {Results/testdataErr.csv};
% \legend{$\mu=0.1$, $\mu=1$, $\mu=10$}
\end{axis}
\end{tikzpicture}
\vspace{0.2cm}
\begin{tikzpicture}[slave,scale=1]
\centering
\begin{axis}[
		width = 0.48\textwidth,
		height = 0.28\textwidth,
 		xmode=normal,
%       xmode=log,
		ymode=normal,	
        xlabel={\large$\eta$},
        ylabel={$q_0(\boldsymbol{x})$},
		ylabel shift = 0cm,
  		xmin=0,
   		xmax=50,
%     	ymin = 10.0,
%      	ymax = 11.5,
%       ytickmax = 11.4,,
%       xtickmax = 7500,
%    xtick={0,2000,4000,6000,,8000},
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\eta \times 10^{-\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
% 		scaled x ticks = base 10:-3,
% 		ytick={10.00, 10.25, 10.50, 10.75, 11.00, 11.25, 11.50},
%     	yticklabels={~, 10.25, 10.50, 10.75, 11.00, 11.25, 11.50},
    	legend pos= north east,
    	ymajorgrids=true,
		xmajorgrids=true,
    	grid style=dashed,
		legend cell align={left},
        legend image post style={scale=0.5},
        legend style={font=\scriptsize, inner xsep=0.2pt, inner ysep=0.1pt, at={(axis cs:49.5,-24)}},
]
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:7.5,-21.2)--(axis cs:49.9,-21.2) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:21.434,-13)--(axis cs:49.9,-13) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.5ex}[0pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:0.958425,-59.5)--(axis cs:49.9,-59.5) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.5ex}[3pt][-0.2ex]{$\mathbf{X}\!=\!\mathbf{x}\mathbf{x}^{\!_\top}$}};
%=========================
\addplot[color=blue,line width=0.5mm] table[x=mu,y=objSDPsdprlt,col sep=comma] {data.csv};
\addplot[dashed,color=red,line width=0.5mm] table[x=mu,y=objSOCPsdprlt,col sep=comma] {data.csv};
\addplot[dash dot,color=black,line width=0.5mm] table[x=mu,y=objSDPRLTsdprlt,col sep=comma] {data.csv};

\legend{$\mathrm{SDP}$,$\mathrm{SOCP}$,$\mathrm{SDP\!+\!RLT}$}
%========================
\end{axis}
\end{tikzpicture}
\vspace{-2mm}
\caption{Sensitivity of the penalized SDP, SOCP, and SDP+RLT relaxations to the choice of penalty parameter $\eta$ for the QCQP benchmark case 1143 and $\hat{\boldsymbol{x}} =\boldsymbol{x}^{\!\!\!\!\!.^{\ast}\;\mathrm{SDP+RLT}}$.}
\label{plt:sdprlt}
\end{figure}
% SDP: 7.67709,4.41813e-12,-34.8958,
% SOCP: 21.334,6.74284e-12,-2.73455,
% SDPRLT: 1.96499,3.2538e-08,-55.761

% 7.67709,1.65604e-11,-54.885
% 21.334,7.07008e-12,-51.1894
% 0.838425,6.33583e-07,-57.1793
